Quantum Communication Complexity of Classical Auctions

We study the fundamental, classical mechanism design problem of single-buyer multi-item Bayesian revenue-maximizing auctions under the lens of communication complexity between the buyer and the seller. Specifically, we ask whether using quantum communication can be more efficient than classical communication. We have two sets of results, revealing a surprisingly rich landscape - which looks quite different from both quantum communication in non-strategic parties, and classical communication in mechanism design. We first study the expected communication complexity of approximately optimal auctions. We give quantum auction protocols for buyers with unit-demand or combinatorial valuations that obtain an arbitrarily good approximation of the optimal revenue while running in exponentially more efficient communication compared to classical approximately optimal auctions. However, these auctions come with the caveat that they may require the seller to charge exponentially large payments from a deviating buyer. We show that this caveat is necessary - we give an exponential lower bound on the product of the expected quantum communication and the maximum payment. We then study the worst-case communication complexity of exactly optimal auctions in an extremely simple setting: additive buyer's valuations over two items. We show the following separations: 1. There exists a prior where the optimal classical auction protocol requires infinitely many bits, but a one-way message of 1 qubit and 2 classical bits suffices. 2. There exists a prior where no finite one-way quantum auction protocol can obtain the optimal revenue. However, there is a barely-interactive revenue-optimal quantum auction protocol. 3. There exists a prior where no multi-round quantum auction protocol with a finite bound on communication complexity can obtain the optimal revenue.

==> newintrocameraready.tex <==

\section{Introduction}

We study the quantum communication complexity of classical problems with strategic constraints. The communication problems we study differ from traditional (``cooperative'') problems in communication complexity like Set Disjointness due to Incentive Compatibility (IC) constraints.
Informally speaking, one can think of the goal of a traditional communication problem is to design   a protocol for both parties that optimizes some common objective function. 

For instance, in Set Disjointness, the common goal is to maximize the probability of outputing the correct answer. 
By contrast, in strategic communication, each party optimizes a different objective; we seek protocols that are communication-efficient, and at the same time don't expect strategic parties to take actions that are mis-aligned with their objectives. 



Specifically, we study the quantum communication complexity of a fundamental setting in mechanism design: a monopolistic, revenue-maximizing seller with Bayesian prior auctioning $n$ items to a single buyer; this setting has proved very attractive to researchers in theoretical computer science (e.g.~\cite{BabaioffILW20, ChenDOPSY15, BabaioffGN22, Gonczarowski18, GuoHZ19, RubinsteinZ21} and references therein).

It is known that even with seemingly benign Bayesian priors, revenue-optimality requires complex auctions, e.g.~ones that allow the buyer to choose among lotteries~\cite{Thanassoulis04,ManelliV10,BriestCKW10,Pavlov11,HartR15}. 
This realization has sparked a fruitful line of work on the simplicity-vs-complexity of  (approximately) optimal auctions. 
Understanding the tradeoffs of simplicity vs.~complexity requires formal definitions of complexity. 

Perhaps the most well-studied notion of complexity for this problem is the number of distinct lotteries offered to the buyer (``menu-size complexity''~\cite{HartN19}). 
The measure exactly characterizes the {\em deterministic communication} complexity of the interaction between a buyer and seller who both know the rules of the auction%
 \footnote{Specifically, $\text{deterministic-CC} = \log\big(\lceil \text{menu-size complexity}\rceil \big)$.}~\cite{BabaioffGN22}.



We study the communication complexity of auctions subject to an Incentive Compatibility (IC) constraint: it is crucial that a strategic buyer must not be able to gain from deviating from the protocol.
(As is standard in the literature, we assume that the seller is non-strategic and follows the protocol faithfully. See Section~\ref{sec:model} for formal definition, and e.g.~\cite{FadelS09,DobzinskiR21,RubinsteinZ21,RubinsteinSTWZ21} for further discussion.)
Under this IC constraint, \cite{RubinsteinZ21} show that it is possible to obtain dramatic savings in communication by considering (classical) {\em randomized communication}. The main question we ask in this work is whether {\em quantum communication} can be even more efficient than classical randomized communication complexity for this problem:

\begin{quote}
    Can quantum auction protocols achieve super-classical performance? 
\end{quote}



Specifically,~\cite{RubinsteinZ21} show that even though randomized auction protocols can be much more efficient than deterministic ones, they  still have limitations:
\begin{itemize}
    \item {\bf Worst-case vs expected CC barrier:} \cite{RubinsteinZ21} improve the communication complexity in expectation (over the randomness of the protocol), but the worst-case communication complexity of randomized protocols is still characterized by the menu-size complexity. 
    \item {\bf Combinatorial valuations barrier:} For buyers with combinatorial valuations over the items, \cite{RubinsteinZ21} prove exponential lower bounds even for the expected communication of randomized auction protocols. These lower bounds hold even for approximately optimal mechanisms, and even against restricted classes of valuations (e.g.~monotone submodular valuations). 
\end{itemize}
In this paper, we investigate to what extent quantum communication can break these classical barriers.


\subsection{Our Contributions}
We formalize a model of {\em quantum auction protocols} (Definition~\ref{def:quantumauction}) that extends the randomized auction protocols of~\cite{RubinsteinZ21} by allowing the buyer and seller to send, receive, operate on, and measure qubits. We then provide two sets of results, centered around the two barriers for classical auction protocols mentioned above.



\subsubsection{(Un)expected Quantum CC with Combinatorial Valuations}
Our first result is an exponential quantum speed-up for auction protocols. It is stated in a general form for a mechanism that chooses an allocation among $B$ possible allocations. Specifically, it gives a near-equivalent IC quantum auction protocol that uses only $O(\log(B))$ qubits --- matching the cost of naively encoding the allocation (without strategic considerations). 
\begin{theorem}[Efficient in-expectation quantum auction protocols]\label{thm:combinatorial-protocol} \hfill

    Let $\cal{D}$ be a prior over buyer's combinatorial valuations over $n$ items; assume all valuations are in the range%
    \footnote{Our protocol assumes that we're given some finite upper bound $U$ on valuations, but the communication complexity does not depend on $U$.} $[0,U]$. 
    Let $\cM$ be any mechanism that can only possibly allocate one of $B$ subsets of the items. Finally, let $\delta > 0$ be any parameter ($\delta$ may be a function of $n$ or $B$). Then there is an IC quantum auction protocol that guarantees a $(1-\delta)$-fraction of $\cM$'s expected revenue using $O(\log(B))$ qubits in expectation.
\end{theorem}
As a corollary, we only need $O(\log(n))$  qubits for unit-demand, or $O(n)$ qubits for arbitrary combinatorial valuations. On the contrary, \cite{RubinsteinZ21} shows that any randomized classical communication protocol requires at least $\Omega(n)$ bits for unit-demand, and  $\Omega(2^n)$ bits for combinatorial valuations.
To the best of our knowledge, this is the first exponential separation of quantum and classical communication in algorithmic game theory.

The positive result in Theorem~\ref{thm:combinatorial-protocol} has a caveat: the protocol may require large payments. Specifically, we need the ability to inflict a large penalty on buyers who deviate from the intended quantum strategy. However, the probability of catching deviating buyers may be exponentially small, so we use exponentially large payments. Even though buyers who follow the protocol can never be penalized, to be accountable for a potentially large payment the buyer may need significant collateral to participate in the auction. 
Our second result shows that unfortunately without exponentially large payments all the lower bounds from~\cite{RubinsteinZ21} extend to quantum communication.

\begin{theorem}[Efficient protocols require large payments - short version] \label{thm:large-payments-intro} \hfill

    Let $n$ be the number of items, $P$ be an upper bound on the payments in the quantum auction protocol (when the valuations are normalized to $[0,1]$), and $\hat{K}$ an upper bound on the expected communication complexity. Then for a buyer with combinatorial (XOS) valuations, any quantum auction protocol that obtains $\Omega(1)$-approximation to the optimal revenue must satisfy $\hat{K} P= 2^{\Omega(n)}$. See Theorem~\ref{thm:large-payments} for full statement and additional results.
\end{theorem}

Interestingly, we are not aware of any classical analogs of such tradeoffs between maximum payment and communication complexity. In particular, the exponential lower bounds against classical auction protocols in~\cite{RubinsteinZ21} hold even with arbitrarily large payments.

\subsubsection{Worst-Case Quantum CC with Two Items}
Our second set of results focuses on the particularly simple case of a buyer with additive valuations over only two items, and the Bayesian prior for these values is independent. In this case, classical protocols of~\cite{RubinsteinZ21} already achieve $O(1)$ expected communication, but their worst-case communication is infinite. Note that this is for exactly optimal mechanisms --- for approximately optimal mechanisms, worst-case can be reduced to expected communication.

We show that on one hand, a {\em single qubit} can sometimes replace an {\em infinite} stream of classical bits. 

\begin{theorem}[Separating one-way quantum vs classical]\label{thm:1-way-protocol} \hfill

    For the problem of auctioning two items to a single buyer, there is a Bayesian prior over independent item values, such that there is a revenue-optimal and IC one-way quantum auction protocol where the buyer sends 1 qubit and 2 classical bits; yet no finite classical auction protocol can achieve the optimal revenue.
\end{theorem}

Furthermore, interactive quantum protocols are even more powerful:

\begin{theorem}[Separating interactive quantum vs one-way quantum]\hfill\label{thm:interactive-vs-1-way}

    For the problem of auctioning two items to a single buyer, there is a Bayesian prior over independent item values, such that there is an IC revenue-optimal quantum auction protocol where the seller sends 1 qubit to the buyer, who replies with 1 qubit and 2 classical bits; yet no finite classical or one-way quantum auction protocol can achieve the optimal revenue.
\end{theorem}

However, in the worst case, even fully interactive quantum auction protocols cannot achieve optimal revenue in finite worst-case communication. 

\begin{theorem}[Limitations of finite interactive quantum auction protocols]\label{thm:non-algebraic}\hfill

    For the problem of auctioning two items to a single buyer, there is a Bayesian prior over independent item values, such that there is a revenue-optimal classical auction protocol that requires a constant number of bits {\em in exepctation}; yet no worst-case finite IC quantum auction protocol can achieve the optimal revenue.
\end{theorem}




\subsection{Key Takeaway: Thinking About Quantum and Incentives Together}\label{sub:quantumplusincentives}


Communication complexity in game-theoretic setting and quantum communication complexity have each been studied extensively over the past few decades, but in separate lines of work, and to a large extent in disjoint communities. The key takeaway from our work is that we can unlock significant advantages by thinking of both together - advantages that are not possible by composing disjoint results for classical-strategic communication and quantum-cooperative communication. 

In particular, it is important to note that our quantum speed-ups are not achievable by a generic quantum speed-up on communication (for example, Holevo's theorem states that an $n$-qubit quantum state, even with infinite precision, can only carry up to $n$ classical bits accessible information \cite{Holevo73}). In fact, they cannot be derived from a quantum speed-up on any non-strategic communication problem. 

We further note that our infinite separations require quantum operations with infinite precision. While this is clearly not practical, it is the standard textbook model of quantum computing, and, to the best of our knowledge, no previous work on quantum-cooperative communication complexity exhibits infinite separations\footnote{ Compared with quantum advantages in interactive proofs,  e.g.~the celebrated $\mathsf{MIP}^* = \mathsf{RE} $~\cite{JNVWY21}, it is worth noting that the latter is only an ``unbounded'' separation, i.e.~that separation still needs the complexity of the $ \mathsf{MIP}^*$ provers to go to infinity. In contrast, we show separation of 3 qubits vs infinitely many classical bits.}.

We highlight some of the ways in which our results are distinct from previous work in either line of work in Figure~\ref{fig:surprise-quantum} and Figure \ref{fig:surprise-AGT}.



\iffalse

\definecolor{softblack}{gray}{0.2}

\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{
 \arrayrulecolor{softblack}
\setlength{\arrayrulewidth}{1pt}
\renewcommand{\arraystretch}{1.5}

\begin{tabular}{|c c|}
\hline
\multicolumn{1}{|c}{ \cellcolor{gray!10} \Large Surprises for quantum} & 
\multicolumn{1}{c|}{ \cellcolor{gray!10} \Large Surprises for AGT} \\
{} \textbf{Infinite 1-way-vs-interactive separation}& {} \textbf{Infinite 1-way-vs-interactive separation} \\
 \textbf{Infinite quantum-classical separation} & \\
{} \textbf{Exp quantum speedup on a natural problem} & {} \textbf{Exp lower bound on CC $\times$ payment} \\

\hline
\end{tabular}
}
\caption{Surprising aspects of our results.}
\label{fig:surprise}
\end{figure}

\begin{figure}
\centering
\resizebox{\columnwidth}{!}{
 \arrayrulecolor{softblack}
\setlength{\arrayrulewidth}{1pt}
\renewcommand{\arraystretch}{1.5}

\begin{tabular}{|c c|}
\hline
\multicolumn{1}{|c}{ \cellcolor{gray!10} \Large Surprising aspects} & 
\multicolumn{1}{c|}{ \cellcolor{gray!10} \Large Surprises for quantum or AGT} \\
{} \textbf{Infinite 1-way-vs-interactive separation}& {} \textbf{Both quantum and AGT} \\
 \textbf{Infinite quantum-classical separation} & \textbf{Quantum} \\
{} \textbf{Exp quantum speedup on a natural problem} & \textbf{Quantum}  \\
\textbf{Exp lower bound on CC $\times$ payment} & \textbf{AGT} \\
\hline
\end{tabular}
}
\caption{Surprising aspects of our results.}
\label{fig:surprise}
\end{figure}

\fi

\begin{figure}[t]
\centering
\begin{tcolorbox}

{\bf Surprises for the quantum side:}
\begin{itemize}
    \item \textbf{Exponential quantum speedup on a natural problem (Theorem~\ref{thm:combinatorial-protocol}).} For combinatorial and unit-demand auctions, we find quantum protocols that are exponentially more efficient than any classical protocol. Existing exponential quantum-classical separations (in cooperative communication complexity) are for problems like Hidden Matching Problem~\cite{BZJK04} that were designed for the purpose of exhibiting a separation. In contrast, the strategic communication problem we study here was considered before in classical algorithmic game theory~\cite{BabaioffGN22, RubinsteinZ21}.

    \item \textbf{Infinite 1-way vs. 1-way + entanglement separation (Theorem~\ref{thm:interactive-vs-1-way}). }%
    Specifically, we show that a one-way protocol with pre-shared entanglement (an EPR pair) is infinitely more efficient than any one-way protocol with no shared entanglement. This unique separation does not exist in the cooperative quantum communication environment as the honest sender can always prepare the EPR pair and send one half through the channel.
    
    \item \textbf{Infinite quantum-classical separation (Theorem~\ref{thm:1-way-protocol}).} We construct an example where we can implement the optimal auction with a one-way quantum communication protocol with $3$ qubits in the worst case. However, no worst-case finite classical protocol can implement it.

\end{itemize}

\end{tcolorbox}

\caption{Summary of most surprising aspects of our results from quantum perspective.}
\label{fig:surprise-quantum}
\end{figure}

\begin{figure}
\centering
\begin{tcolorbox}



{\bf Surprises for the AGT side:}
\begin{itemize}
    \item \textbf{Infinite 1-way vs. interactive separation (Theorem~\ref{thm:interactive-vs-1-way}).} 
    We show an example where an interactive two-way quantum protocol is infinitely better than any one-way quantum protocol. This unique separation does not exist in the classical setting. Since with a trusted party (the seller in our setting), any classical protocol can be ``flattened'' to a one-way protocol incurring an exponential overhead in the worst-case communication complexity, yet this overhead remains finite.
    \item \textbf{Exponential lower bound on CC $\times$ payment (Theorem~\ref{thm:large-payments}).} We prove that our exponentially more efficient quantum protocol in Theorem~\ref{thm:combinatorial-protocol} necessitates an exponentially large payment, by establishing an exponential lower bound on the product of payment and communication complexity. This characteristic is distinctive to the quantum setting, as the exponential lower bounds for classical protocols~\cite{RubinsteinZ21} apply even with arbitrarily large payments.
    
\end{itemize}


\end{tcolorbox}

\caption{Summary of most surprising aspects of our results from AGT perspective.}
\label{fig:surprise-AGT}
\end{figure}





% \jack{do we want to elaborate on these bullets?}

\paragraph*{Core conceptual idea: Efficient, samplable and verifiable distribution encodings.}
At a high level, the communication protocol of Bayesian auction boils down to the following task: The seller has a set $\mathcal{S}$ consisting of valid distributions of auction outcomes (allocation and payment). The buyer then selects a distribution $D$ from $\mathcal{S}$ that maximizes his utility. Subsequently, the seller draws a sample from the chosen distribution $D$ and outputs it as the outcome. In general, the complexity of describing a distribution is exponentially higher than specifying an outcome. It is worth noting that this task is completely trivial in a fully cooperative environment as the buyer can simply draw the outcome himself and send only this outcome to the seller. A natural quantum solution to this problem is that the buyer can efficiently encode $D$ in state $\sum_{x} \sqrt{D_x} \ket{x}$. To draw an element from the distribution, the seller only needs to measure this quantum state in the computational basis. However, this simple approach has a caveat -- in general it is information theoretically impossible for the seller to verify that this quantum state indeed encodes a valid distribution in set $\mathcal{S}$. To overcome this issue, our paper proposes two solutions. The first one is a general spot-check method -- with a small probability, after receiving the quantum state, the seller asks the buyer to send the whole classical description of the distribution; the seller verifies that the classical description is valid and the quantum state is close enough to this classical description. By imposing an exponentially large penalty, we ensure that the buyer is always incentivized to prepare a quantum state corresponding to a valid distribution while keeping the {\em expected} communication complexity low. The other solution works for the worst case communication complexity under some specific assumptions on the set of valid distribution of auction outcomes. These assumptions are satisfied for example by the canonical classically-hard example of~\cite{DaskalakisDT17}, but not in general (see Theorem~\ref{thm:non-algebraic}).  By carefully tailoring the quantum protocol to the desired auction, we can ensure that the space of distributions that the buyer can encode  coincides with the desired valid space.


\subsection{Additional Related Works}\label{sub:related}
Our work extends a rich tradition of studying mechanism design and game theory under the lens of communication complexity --- including auctions~\cite{NisanS06,BlumrosenNS07,BabaioffBS13,DobzinskiV13,DobzinskiNO14,Dobzinski16a,Dobzinski16b,BravermanMW16,Assadi17,BravermanMW18,EzraFNTW19,AssadiKSW20,BabaioffGN22, WeinbergZ22}, and also stable matching~\cite{GonczarowskiNOR19}, voting rules~\cite{ConitzerS05,ProcacciaR06a,CaragiannisP11,ServiceA12a},
 fair division~\cite{BranzeiN19,PlautR19}, computation of equilibria~\cite{ConitzerS04,HartM10,RoghgardenW16,GoosR18,GanorS18,BabichenkoDN19,BabichenkoR20,GanorSP21,BabichenkoR22}, and interdomain routing~\cite{LSZ11}. In particular, the communication complexity of IC implementing a mechanism  vs that of (non-IC) computing the outcome was the focus of~\cite{FadelS09,DobzinskiR21,RubinsteinSTWZ21,DobzinskiRV22}.



We show exponential separations (and for worst-case complexity --- infinite separations) between quantum and classical communication complexity of auctions. Earlier works on separating the two measures (in non-strategic settings) include
general boolean functions (constructed for obtaining separations)~\cite{ Raz99, BZJK04, Gav08, GKKRdW09, RegevK11}, sampling~\cite{ASTAVW03, Montanaro19}, and very recently also linear regression~\cite{MontanaroS22, TLWXH+22}.


Our work is also related to works on quantum game theory --- including nonlocal games~\cite{CHSH69, CHTW04}, quantization of classical games~\cite{EWL99, Meyer00}, quantum equilibria~\cite{Deckelbaum11, WeiZ13}, and quantum interactive games~\cite{GutoskiW07}. In particular, quantum interactive strategies are also studied in quantum interactive proofs~\cite{Watrous03, BSW10, JJUW10, NW19, JNVWY21}.

%TBD compare 


\subsection{Organization}
We begin with a review of the quantum communication model and mechanism design in Section~\ref{sec:prelim-quantum} and \ref{sec:prelim-MD}, and then introduce our main model of quantum auction protocols in Section~\ref{sec:model}. Part~\ref{part:combinatorial} brings our results for expected communication: Our quantum auction protocol for combinatorial valuations in Section~\ref{sec:eps-IC-protocol}, and our lower bound against quantum auction protocols with bounded maximum payment in Section~\ref{sec:small-payments}. Part~\ref{part:2-items} focuses on worst-case communication: we begin with preliminaries of optimal 2-item auctions in Section~\ref{sec:prelim-2-items}; in Section~\ref{sec:1-way-protocol} we construct an example separating one-way quantum auction protocols from finite classical; in Sections~\ref{sec:limit-1-way} and~\ref{sec:barely-interactive} we separate interactive quantum auction protocols from one-way; and finally in Section~\ref{sec:finite-round} we show that in general no finite quantum auction protocol can guarantee optimal revenue. 



